Bicategories of fractions revisited: towards small homs and canonical 2-cells

This paper adresses two issues in dealing with bicategories of fractions. The first is to introduce a set of conditions on a class of arrows in a bicategory which is weaker than the one given in Pronk, Etendues and stacks as bicategories of fractions, but still allows a bicalculus of fractions. These conditions allow us to invert a smaller collection of arrows so that in some cases we may obtain a bicategory of fractions with small hom-categories. We adapt the construction of the bicategory of fractions to work with the weaker conditions. The second issue is the difficulty in dealing with 2-cells, which are defined by equivalence classes. We discuss conditions under which there are canonical representatives for 2-cells, and how pasting of 2-cells can be simplified in the presence of certain pseudo pullbacks. We also discuss how both of these improvements apply in the category of orbispaces.

==> horizontalcomp_proof.tex <==
\section{Horizontal Composition of 2-Cell Diagrams}\label{horcomp}

In this appendix we provide a proof for the following result, described in Section \ref{horcomppb}:

\begin{prop}
If $\frakW$ in the bicategory $\calB$ is pullback-closed, satisfies the fractions axioms and is co-full, the horizontal composition of the composable 2-cell diagrams in (\ref{composable-2-cells}) of Section \ref{horcomppb} for the category of fractions $\calB(\frakW^{-1})$ can be represented by the 2-cell diagram in (\ref{horcomposition}).
\end{prop}

\begin{proof}
We construct the horizontal composition of the 2-cell diagrams of (\ref{composable-2-cells})  using whiskering and vertical composition:
$$([\rho_{v_1,v_2},\gamma](f_2,u_2))\cdot((v_1,g_1)[\rho_{u_1,u_2},\beta])$$
We start by considering the whiskering $((v_1,g_1)[\rho_{u_1,u_2},\beta])$.  To construct this, we need the chosen square:  
$$
\xymatrix@R=2.5em@C=2.5em{
\ar[r]^{v_1^*}\ar[d]_{f_2^*} \ar@{}[dr]|{\Downarrow\varepsilon_{1,2}}& \ar[d]^{f_2}
\\
\ar[r]_{v_1}&
}
$$
This lets us construct the horizontal composition of the arrows as in the following diagram (which is not a pasting diagram):
% https://q.uiver.app/?q=WzAsMTUsWzIsMiwiUF97dV8xLHVfMn0iXSxbMiwxXSxbMCwyLCJBIl0sWzIsM10sWzQsMiwiQiJdLFs2LDIsIkInIl0sWzQsMSwiXFxEb3duYXJyb3dcXGRlbHRhXzEiXSxbNCwzLCJcXERvd25hcnJvd1xcdmFyZXBzaWxvbl97MSwyfV57LTF9Il0sWzgsMiwiQyJdLFsxLDIsIlxccmhvX3t1XzEsdV8yfVxcRG93bmFycm93Il0sWzMsMiwiXFxiZXRhXFxEb3duYXJyb3ciXSxbMiw0LCJBJyciXSxbMiwwLCJBJyJdLFs0LDQsIkReKiJdLFs0LDAsIkQiXSxbNSw0LCJ2XzEiLDFdLFs1LDgsImdfMSJdLFswLDExLCJcXHBpX3tBJyd9IiwxXSxbMCwxMiwiXFxwaV97QSd9IiwxXSxbMTIsMiwidV8xIiwyXSxbMTEsMiwidV8yIl0sWzEzLDExLCJ2XzFeKiJdLFsxMyw1LCJmXzJeKiIsMV0sWzE0LDUsIlxcb3ZlcmxpbmV7Zn1fMSIsMV0sWzE0LDEyLCJcXG92ZXJsaW5le3Z9XzEiLDJdLFsxMiw0LCJmXzEiLDFdLFsxMSw0LCJmXzIiLDFdXQ==
\[\begin{tikzcd}[column sep=small, row sep = small]
	&& {A'} && D \\
	&& {} && {\Downarrow\delta_1} \\
	A & {\rho_{u_1,u_2}\Downarrow} & {P_{u_1,u_2}} & \beta\Downarrow & B && {B'} && C \\
	&& {} && {\Downarrow\varepsilon_{1,2}^{-1}} \\
	&& {A''} && {D^*}
	\arrow["{v_1}"{description}, from=3-7, to=3-5]
	\arrow["{g_1}", from=3-7, to=3-9]
	\arrow["{\pi_{A''}}"{description}, from=3-3, to=5-3]
	\arrow["{\pi_{A'}}"{description}, from=3-3, to=1-3]
	\arrow["{u_1}"', from=1-3, to=3-1]
	\arrow["{u_2}", from=5-3, to=3-1]
	\arrow["{v_1^*}", from=5-5, to=5-3]
	\arrow["{f_2^*}"{description}, from=5-5, to=3-7]
	\arrow["{\overline{f}_1}"{description}, from=1-5, to=3-7]
	\arrow["{\overline{v}_1}"', from=1-5, to=1-3]
	\arrow["{f_1}"{description}, from=1-3, to=3-5]
	\arrow["{f_2}"{description}, from=5-3, to=3-5]
\end{tikzcd}\]
To construct the 2-cells involved in the whiskering $(v_1,g_1) [\rho_{u_1,u_2},\beta]$ we will use the pseudo-pullback square
$$
\xymatrix@C=4.5em{
P_{u_1\overline{v}_1,u_2v_1^*} \ar[d]_{\pi'_{D^*}} \ar[r]^{\pi'_D} \ar@{}[dr]|{\wr\Downarrow\rho_{u_1\overline{v}_1,u_2v_1^*}} & D \ar[d]^{u_1\overline{v}_1}
\\
D^*\ar[r]_{u_2v_1^*} &A}
$$
Let $w^*_{u_1,u_2}\colon P_{u_1\overline{v}_1,u_2v_1^*} \rightarrow P_{u_1,u_2}$ be the unique arrow such that
$\rho_{u_1,u_2}w^*_{u_1,u_2}=\rho_{u_1\overline{v}_1,u_2v_1^*}$.
Then the whiskering of $[\rho_{u_1,u_2},\beta]$ with $(v_1,g_1)$ can be obtained by considering diagram below and then taking a lifting with respect to $v_1$:
% https://q.uiver.app/?q=WzAsMTAsWzMsMSwiQSciXSxbMywyLCJQX3t1XzEsdV8yfSJdLFszLDMsIkEnJyJdLFsyLDQsIkReKiJdLFsyLDIsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJ2XzFeKn0iXSxbNCwyLCJCIl0sWzUsMiwiQiciXSxbMCwyLCJBIl0sWzYsMiwiQyJdLFsyLDAsIkQiXSxbMSwwLCJcXHBpX3tBJ30iXSxbMSwyLCJcXHBpX3tBJyd9IiwyXSxbMywyLCJ2XzFeKiIsMV0sWzQsMywiXFxwaV97RF4qfSIsMl0sWzAsNSwiZl8xIiwxXSxbMiw1LCJmXzIiLDFdLFs2LDUsInZfMSJdLFszLDYsImZfMl4qIiwyLHsiY3VydmUiOjV9XSxbMyw3LCJ1XzJ2XzFeKiIsMCx7ImN1cnZlIjotMX1dLFs2LDgsImdfMSIsMl0sWzQsOSwiXFxwaV9EIl0sWzksMCwiXFxvdmVybGluZXt2fV8xIiwxXSxbOSw2LCJcXG92ZXJsaW5le2Z9XzEiLDAseyJjdXJ2ZSI6LTV9XSxbOSw3LCJ1XzFcXG92ZXJsaW5le3Z9XzEiLDIseyJjdXJ2ZSI6MX1dLFs0LDEsIndeKl97dV8xLHVfMn0iXSxbMTUsMTcsIlxcdmFyZXBzaWxvbl97MTJ9XnstMX0iLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MzAsInRhcmdldCI6MzB9fV0sWzIzLDE4LCJcXHJob197dV8xXFxvdmVybGluZXt2fV8xLHVfMnZfMV4qfSIsMSx7InNob3J0ZW4iOnsic291cmNlIjozMCwidGFyZ2V0IjozMH19XSxbMTQsMTUsIlxcYmV0YSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XSxbMjIsMTQsIlxcZGVsdGFfMSIsMCx7InNob3J0ZW4iOnsic291cmNlIjozMCwidGFyZ2V0IjozMH19XSxbMjQsMTIsIiIsMSx7InNob3J0ZW4iOnsic291cmNlIjo0MCwidGFyZ2V0Ijo0MH0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjEsMjQsIiIsMSx7InNob3J0ZW4iOnsic291cmNlIjo0MCwidGFyZ2V0Ijo0MH0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\begin{equation}\label{first-2-cell}\begin{tikzcd}[ampersand replacement=\&]
	\&\& D \\
	\&\&\& {A'} \\
	A \&\& {P_{u_1\overline{v}_1,u_2v_1^*}} \& {P_{u_1,u_2}} \& B \& {B'} \& C \\
	\&\&\& {A''} \\
	\&\& {D^*}
	\arrow["{\pi_{A'}}", from=3-4, to=2-4]
	\arrow["{\pi_{A''}}"', from=3-4, to=4-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{v_1^*}"{description}, from=5-3, to=4-4]
	\arrow["{\pi'_{D^*}}"', from=3-3, to=5-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{f_1}"{description}, from=2-4, to=3-5]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{f_2}"{description}, from=4-4, to=3-5]
	\arrow["{v_1}", from=3-6, to=3-5]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{f_2^*}"', curve={height=30pt}, from=5-3, to=3-6]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{u_2v_1^*}", curve={height=-6pt}, from=5-3, to=3-1]
	\arrow["{g_1}"', from=3-6, to=3-7]
	\arrow["{\pi'_D}", from=3-3, to=1-3]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{\overline{v}_1}"{description}, from=1-3, to=2-4]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\overline{f}_1}", curve={height=-30pt}, from=1-3, to=3-6]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{u_1\overline{v}_1}"', curve={height=6pt}, from=1-3, to=3-1]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{w^*_{u_1,u_2}}", from=3-3, to=3-4]
	\arrow["{\varepsilon_{12}^{-1}}", shorten <=9pt, shorten >=9pt, Rightarrow, from=2, to=3]
	\arrow["{\rho_{u_1\overline{v}_1,u_2v_1^*}}"{description}, shorten <=15pt, shorten >=15pt, Rightarrow, from=7, to=4]
	\arrow["\beta"{description}, shorten <=4pt, shorten >=4pt, Rightarrow, from=1, to=2]
	\arrow["{\delta_1}", shorten <=9pt, shorten >=9pt, Rightarrow, from=6, to=1]
	\arrow[shorten <=13pt, shorten >=13pt, Rightarrow, no head, from=8, to=0]
	\arrow[shorten <=13pt, shorten >=13pt, Rightarrow, no head, from=5, to=8]
\end{tikzcd}\end{equation}
Once we create a 2-cell by lifting the right-hand pasting diagram from above, we write this 2-cell as  $\tilde\beta$.  We obtain then the following 2-cell diagram in the bicategory of fractions:
% https://q.uiver.app/?q=WzAsNixbMCwxLCJBIl0sWzIsMCwiRCJdLFsyLDIsIkReKiJdLFsyLDEsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJ2XzFeKn0iXSxbNCwxLCJCJyJdLFs2LDEsIkMiXSxbMiwwLCJ1XzJ2XzFeKiJdLFsxLDAsInVfMVxcb3ZlcmxpbmV7dn1fMSIsMl0sWzMsMSwiXFxwaV9EIl0sWzMsMiwiXFxwaV97RF4qfSIsMl0sWzQsNSwiZ18xIl0sWzEsNCwiXFxvdmVybGluZXtmfV8xIl0sWzIsNCwiZl8yXioiLDJdLFs3LDYsIlxccmhvX3t1XzFcXG92ZXJsaW5le3Z9XzEsdV8ydl8xXip9IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxMSwxMiwiXFx0aWxkZVxcYmV0YSIsMix7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XV0=
\[\begin{tikzcd}[ampersand replacement=\&]
	\&\& D \\
	A \&\& {P_{u_1\overline{v}_1,u_2v_1^*}} \&\& {B'} \&\& C \\
	\&\& {D^*}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{u_2v_1^*}", from=3-3, to=2-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{u_1\overline{v}_1}"', from=1-3, to=2-1]
	\arrow["{\pi'_D}", from=2-3, to=1-3]
	\arrow["{\pi'_{D^*}}"', from=2-3, to=3-3]
	\arrow["{g_1}", from=2-5, to=2-7]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\overline{f}_1}", from=1-3, to=2-5]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{f_2^*}"', from=3-3, to=2-5]
	\arrow["{\rho_{u_1\overline{v}_1,u_2v_1^*}}"{description}, shorten <=4pt, shorten >=4pt, Rightarrow, from=1, to=0]
	\arrow["\tilde\beta"', shorten <=4pt, shorten >=4pt, Rightarrow, from=2, to=3]
\end{tikzcd}\]
Now we consider the other half of the composition, the whiskering
$[\rho_{v_1,v_2},\gamma](u_2,f_2)$.
The domain and codomain arrows for the whiskering are constructed in the following diagram (not a pasting diagram):
% https://q.uiver.app/?q=WzAsOSxbNiwxLCJQX3t2XzEsdl8yfSJdLFs2LDAsIkInIl0sWzYsMiwiQicnIl0sWzQsMSwiQiJdLFs4LDEsIkMiXSxbMiwxLCJBJyciXSxbMCwxLCJBIl0sWzQsMCwiRF4qIl0sWzQsMiwiRCciXSxbMCwxLCJcXHBpX3tCJ30iLDJdLFswLDIsIlxccGlfe0InJ30iXSxbMSwzLCJ2XzEiLDFdLFsyLDMsInZfMiIsMV0sWzEsNCwiZ18xIl0sWzIsNCwiZ18yIiwyXSxbNSwzLCJmXzIiLDFdLFs1LDYsInVfMiIsMV0sWzcsMSwiZl8yXioiLDFdLFs3LDUsInZfMV4qIiwxXSxbOCwyLCJcXG92ZXJsaW5le2Z9XzIiLDFdLFs4LDUsIlxcb3ZlcmxpbmV7dn1fMiIsMV0sWzExLDEyLCJcXHJob197dl8xLHZfMn0iLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzEzLDE0LCJcXGdhbW1hIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxNSwxNywiXFx2YXJlcHNpbG9uX3sxLDJ9IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxOSwxNSwiXFxkZWx0YV8yIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dXQ==
\[\begin{tikzcd}[ampersand replacement=\&]
	\&\&\&\& {D^*} \&\& {B'} \\
	A \&\& {A''} \&\& B \&\& {P_{v_1,v_2}} \&\& C \\
	\&\&\&\& {D'} \&\& {B''}
	\arrow["{\pi_{B'}}"', from=2-7, to=1-7]
	\arrow["{\pi_{B''}}", from=2-7, to=3-7]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{v_1}"{description}, from=1-7, to=2-5]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{v_2}"{description}, from=3-7, to=2-5]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{g_1}", from=1-7, to=2-9]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{g_2}"', from=3-7, to=2-9]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{f_2}"{description}, from=2-3, to=2-5]
	\arrow["{u_2}"{description}, from=2-3, to=2-1]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{f_2^*}"{description}, from=1-5, to=1-7]
	\arrow["{v_1^*}"{description}, from=1-5, to=2-3]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\overline{f}_2}"{description}, from=3-5, to=3-7]
	\arrow["{\overline{v}_2}"{description}, from=3-5, to=2-3]
	\arrow["{\rho_{v_1,v_2}}", shorten <=4pt, shorten >=4pt, Rightarrow, from=0, to=1]
	\arrow["\gamma"', shorten <=4pt, shorten >=4pt, Rightarrow, from=2, to=3]
	\arrow["{\varepsilon_{1,2}}"{description}, shorten <=13pt, shorten >=13pt, Rightarrow, from=4, to=5]
	\arrow["{\delta_2}"{description}, shorten <=13pt, shorten >=13pt, Rightarrow, from=6, to=4]
\end{tikzcd}\]
To find the 2-cell for this whiskering,  we start with the pseudo pullback,
$$
\xymatrix{P_{u_2v_1^*,u_2\overline{v}_2}\ar[rr]^{\pi_{D^*}''}\ar[dd]_{\pi_{D'}''}\ar@{}[ddrr]|{\wr\Downarrow\rho_{u_2v_1^*,u_2\overline{v}_2}} &&D^*\ar[d]^{v_1^*}
\\
&&A''\ar[d]^{u_2}
\\
D'\ar[r]_{\overline{v}_2}&A''\ar[r]_{u_2} &A
}
$$
Let 
$$\xymatrix@C=3.5em@R=3.5em{P_{u_2v_1^*,u_2\overline{v}_2} \ar[r]^{\pi_{D^*}''}\ar[d]_{\pi_{D'}''}\ar@{}[dr]|{\wr\Downarrow\tilde\rho_{u_2v_1^*,u_2\overline{v}_2}} &D^*\ar[d]^{v_1^*}
\\
D'\ar[r]_{\overline{v}_2}&A''
}
$$
be the lifting of this diagram with respect to $u_2$, and let $x_{v_1,v_2}\colon P_{u_2v_1^*,u_2\overline{v}_2}\to P_{v_1,v_2}$ be the unique arrow such that the following equality of  pasting diagrams holds:
% https://q.uiver.app/?q=WzAsMTIsWzAsMiwiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFsyLDIsIlBfe3ZfMSx2XzJ9Il0sWzIsMCwiQiciXSxbMiw0LCJCJyciXSxbNCwyLCJCIl0sWzUsMiwiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFs2LDAsIkReKiJdLFs2LDQsIkQnIl0sWzcsMiwiQScnIl0sWzksMiwiQiJdLFs4LDAsIkInIl0sWzgsNCwiQicnIl0sWzAsMSwieF97dl8xLHZfMn0iXSxbMSwyLCJcXHBpX3tCJ30iXSxbMCwyLCJmXzJeKlxccGlfe0ReKn0nIiwwLHsiY3VydmUiOi0yfV0sWzEsMywiXFxwaV97QicnfSIsMl0sWzAsMywiXFxvdmVybGluZXtmfV8yXFxwaV97RCd9IiwyLHsiY3VydmUiOjJ9XSxbMiw0LCJ2XzEiLDAseyJjdXJ2ZSI6LTJ9XSxbMyw0LCJ2XzIiLDIseyJjdXJ2ZSI6Mn1dLFs1LDYsIlxccGlfe0ReKn0iLDAseyJjdXJ2ZSI6LTF9XSxbNSw3LCJcXHBpX3tEJ30iLDIseyJjdXJ2ZSI6MX1dLFs2LDgsInZfMV4qIiwyXSxbNyw4LCJcXG92ZXJsaW5le3Z9XzIiXSxbOCw5LCJmXzIiXSxbNiwxMCwiZl8yXioiXSxbNywxMSwiXFxvdmVybGluZXtmfV8yIiwyXSxbMTEsOSwidl8yIiwyXSxbMTAsOSwidl8xIl0sWzQsNSwiXFxlcXVpdiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNCwxMiwiIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNiwxMiwiIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxNywxOCwiXFxyaG9fe3ZfMSx2XzJ9IiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxOSwyMCwiXFx0aWxkZXtcXHJob31fe3VfMnZfMV4qLHVfMlxcb3ZlcmxpbmV7dn1fMn0iLDAseyJvZmZzZXQiOi01LCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzI0LDIzLCJcXHZhcmVwc2lsb25fezEsMn0iLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzIzLDI1LCJcXGRlbHRhXzIiLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV1d
\[\begin{tikzcd}[ampersand replacement=\&, column sep = small]
	\&\& {B'} \&\&\&\& {D^*} \&\& {B'} \\
	\\
	{P_{u_2v_1^*,u_2\overline{v}_2}} \&\& {P_{v_1,v_2}} \&\& B \& {P_{u_2v_1^*,u_2\overline{v}_2}} \&\& {A''} \&\& B \\
	\\
	\&\& {B''} \&\&\&\& {D'} \&\& {B''}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{x_{v_1,v_2}}", from=3-1, to=3-3]
	\arrow["{\pi_{B'}}", from=3-3, to=1-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{f_2^*\pi_{D^*}''}", curve={height=-12pt}, from=3-1, to=1-3]
	\arrow["{\pi_{B''}}"', from=3-3, to=5-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\overline{f}_2\pi_{D'}''}"', curve={height=12pt}, from=3-1, to=5-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{v_1}", curve={height=-12pt}, from=1-3, to=3-5]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{v_2}"', curve={height=12pt}, from=5-3, to=3-5]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{\pi_{D^*}''}", curve={height=-6pt}, from=3-6, to=1-7]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\pi_{D'}''}"', curve={height=6pt}, from=3-6, to=5-7]
	\arrow["{v_1^*}"', from=1-7, to=3-8]
	\arrow["{\overline{v}_2}", from=5-7, to=3-8]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{f_2}", from=3-8, to=3-10]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{f_2^*}", from=1-7, to=1-9]
	\arrow[""{name=9, anchor=center, inner sep=0}, "{\overline{f}_2}"', from=5-7, to=5-9]
	\arrow["{v_2}"', from=5-9, to=3-10]
	\arrow["{v_1}", from=1-9, to=3-10]
	\arrow["\equiv"{description}, draw=none, from=3-5, to=3-6]
	\arrow[shorten <=6pt, shorten >=6pt, Rightarrow, no head, from=1, to=0]
	\arrow[shorten <=6pt, shorten >=6pt, Rightarrow, no head, from=2, to=0]
	\arrow["{\rho_{v_1,v_2}}"', shorten <=11pt, shorten >=11pt, Rightarrow, from=3, to=4]
	\arrow["{\tilde{\rho}_{u_2v_1^*,u_2\overline{v}_2}}", shift left=5, shorten <=9pt, shorten >=9pt, Rightarrow, from=5, to=6]
	\arrow["{\varepsilon_{1,2}}", shorten <=10pt, shorten >=10pt, Rightarrow, from=8, to=7]
	\arrow["{\delta_2^{-1}}", shorten <=10pt, shorten >=10pt, Rightarrow, from=7, to=9]
\end{tikzcd}\]
The whiskering $[\rho_{v_1,v_2},\gamma] (u_2,f_2)$ can now be represented by the diagram
\begin{equation}\label{sec-2-cell}
\xymatrix@C=6em{&D^*\ar[r]^{f_2^*}\ar@{}[dr]|= \ar[dl]_{u_2v_1^*}& B'\ar[dr]^{g_1}
\\
A\ar@{}[r]|{\Downarrow\rho_{u_2v_1^*,u_2\overline{v}_2}}&P_{u_2v_1^*,u_2\overline{v}_2} \ar[u]_{\pi''_{D^*}}\ar[d]^{\pi''_{D'}}\ar[r]^{x_{v_1,v_2}}\ar@{}[dr]|= & P_{v_1,v_2}\ar[u]^{\pi_{B'}}\ar[d]_{\pi_{B''}}\ar@{}[r]|{\Downarrow\gamma}&C
\\
&D'\ar[ul]^{u_2\overline{v}_2}\ar[r]_{\overline{f}_2} & B''\ar[ur]_{g_2}
}
\end{equation}

We now want to construct the vertical composition of whiskerings  $([\rho_{v_1,v_2},\gamma](f_2,u_2))$ and $((v_1,g_1)[\rho_{u_1,u_2},\beta])$ as presented in  (\ref{first-2-cell}) and (\ref{sec-2-cell}). For this we need the following pseudo pullback (or any square that commutes up to an invertible 2-cell):
$$
\xymatrix{R\ar[r]^{\pi_1}\ar[d]_{\pi_2}\ar@{}[dr]|{\rho} &P_{u_1\overline{v}_1,\overline{v}_2v_1^*}\ar[d]^{\pi'_{D^*}}\\P_{u_2v_1^*,u_2\overline{v}_2}\ar[r]_{\pi''_{D^*}} & D^*}
$$
Furthermore, let $r\colon R\to P_{u_1\overline{v}_1,u_2\overline{v}_2}$ be the unique arrow such that the following equality of pasting diagrams holds,
% https://q.uiver.app/?q=WzAsMTIsWzAsMiwiUiJdLFsyLDIsIlBfe3VfMVxcb3ZlcmxpbmV7dl8xfSx1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzIsMCwiRCJdLFsyLDQsIkQnIl0sWzQsMiwiQSJdLFs1LDIsIlIiXSxbNiwxLCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsXFxvdmVybGluZXt2fV8ydl8xXip9Il0sWzYsMywiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFs2LDAsIkQiXSxbNywyLCJEXioiXSxbOSwyLCJBIl0sWzYsNCwiRCciXSxbMCwxLCJyIiwxXSxbMSwyLCJcXHBpX0QiXSxbMSwzLCJcXHBpX3tEJ30iLDJdLFswLDMsIlxccGlfe0QnfXIiLDIseyJjdXJ2ZSI6MX1dLFswLDIsIlxccGlfRHIiLDAseyJjdXJ2ZSI6LTF% https://q.uiver.app/?q=WzAsMTIsWzAsMiwiUiJdLFsyLDIsIlBfe3VfMVxcb3ZlcmxpbmV7dl8xfSx1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzIsMCwiRCJdLFsyLDQsIkQnIl0sWzQsMiwiQSJdLFs1LDIsIlIiXSxbNiwxLCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsXFxvdmVybGluZXt2fV8ydl8xXip9Il0sWzYsMywiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFs2LDAsIkQiXSxbNywyLCJEXioiXSxbOSwyLCJBIl0sWzYsNCwiRCciXSxbMCwxLCJyIiwxXSxbMSwyLCJcXHBpX0QiXSxbMSwzLCJcXHBpX3tEJ30iLDJdLFswLDMsIlxccGlfe0QnfXIiLDIseyJjdXJ2ZSI6MX1dLFswLDIsIlxccGlfRHIiLDAseyJjdXJ2ZSI6LTF9XSxbMiw0LCJ1XzFcXG92ZXJsaW5le3Z9XzEiLDAseyJjdXJ2ZSI6LTJ9XSxbMyw0LCJ1XzJcXG92ZXJsaW5le3Z9XzIiLDIseyJjdXJ2ZSI6Mn1dLFs0LDUsIlxcZXF1aXYiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSw2LCJcXHBpXzEiXSxbNSw3LCJcXHBpXzIiLDJdLFs2LDgsIlxccGlfRCciXSxbNiw5LCJcXHBpX3tEXip9IiwxXSxbNyw5LCJcXHBpJ197RF4qfSIsMV0sWzksMTAsInVfMnZfMV4qIiwxXSxbOCwxMCwidV8xXFxvdmVybGluZXt2fV8xIiwwLHsiY3VydmUiOi0yfV0sWzcsMTEsIlxccGknX3tEJ30iLDJdLFsxMSwxMCwidV8yXFxvdmVybGluZXt2fV8yIiwyLHsiY3VydmUiOjJ9XSxbMTYsMTIsIiIsMCx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTIsMTUsIiIsMCx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTcsMTgsIlxccmhvIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsyMCwyMSwiXFxyaG8iLDAseyJvZmZzZXQiOi01LCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzI2LDI1LCJcXHJob197dV8xXFxvdmVybGluZXt2fV8xLFxcb3ZlcmxpbmV7dn1fMnZfMV4qfSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XSxbMjUsMjgsIlxccmhvX3t1XzJ2XzFeKix1XzIsXFxvdmVybGluZXt2fV8yfSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XV0=
\[\begin{tikzcd}[ampersand replacement=\&,column sep = small]
	\&\& D \&\&\&\& D \\
	\&\&\&\&\&\& {P_{u_1\overline{v}_1,\overline{v}_2v_1^*}} \\
	R \&\& {P_{u_1\overline{v_1},u_2\overline{v}_2}} \&\& A \& R \&\& {D^*} \&\& A \\
	\&\&\&\&\&\& {P_{u_2v_1^*,u_2\overline{v}_2}} \\
	\&\& {D'} \&\&\&\& {D'}
	\arrow[""{name=0, anchor=center, inner sep=0}, "r"{description}, from=3-1, to=3-3]
	\arrow["{\pi_D}", from=3-3, to=1-3]
	\arrow["{\pi_{D'}}"', from=3-3, to=5-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi_{D'}r}"', curve={height=6pt}, from=3-1, to=5-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\pi_Dr}", curve={height=-6pt}, from=3-1, to=1-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{u_1\overline{v}_1}", curve={height=-12pt}, from=1-3, to=3-5]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{u_2\overline{v}_2}"', curve={height=12pt}, from=5-3, to=3-5]
	\arrow["\equiv"{description}, draw=none, from=3-5, to=3-6]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{\pi_1}", from=3-6, to=2-7]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\pi_2}"', from=3-6, to=4-7]
	\arrow["{\pi_D'}", from=2-7, to=1-7]
	\arrow["{\pi_{D^*}'}"', from=2-7, to=3-8]
	\arrow["{\pi''_{D^*}}", from=4-7, to=3-8]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{u_2v_1^*}"{description}, from=3-8, to=3-10]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{u_1\overline{v}_1}", curve={height=-12pt}, from=1-7, to=3-10]
	\arrow["{\pi''_{D'}}"', from=4-7, to=5-7]
	\arrow[""{name=9, anchor=center, inner sep=0}, "{u_2\overline{v}_2}"', curve={height=12pt}, from=5-7, to=3-10]
	\arrow[shorten <=5pt, shorten >=5pt, Rightarrow, no head, from=2, to=0]
	\arrow[shorten <=5pt, shorten >=5pt, Rightarrow, no head, from=0, to=1]
	\arrow["{\rho_{u_1\overline{v}_1,u_2\overline{v}_2}}"{description}, shorten <=11pt, shorten >=11pt, Rightarrow, from=3, to=4]
	\arrow["\rho", shift left=5, shorten <=4pt, shorten >=4pt, Rightarrow, from=5, to=6]
	\arrow["{\rho_{u_1\overline{v}_1,\overline{v}_2v_1^*}}"{description}, shorten <=6pt, shorten >=6pt, Rightarrow, from=8, to=7]
	\arrow["{\rho_{u_2v_1^*,u_2,\overline{v}_2}}"{description}, shorten <=6pt, shorten >=6pt, Rightarrow, from=7, to=9]
\end{tikzcd}\]
Now let 
$$
\xymatrix{
&D\ar[dr]^{g_1\overline{f}_1}\ar@{}[dd]|{\widetilde{\beta\gamma}}
\\
P_{u_1\overline{v}_1,u_2\overline{v}_2} \ar[ur]^{\pi_D} \ar[dr]_{\pi_{D'}} && C
\\
&D'\ar[ur]_{g_2\overline{f}_2}
}
$$
be a lifting with respect to $r$ of the pasting of the following diagram,
% https://q.uiver.app/?q=WzAsMTIsWzAsMCwiUF97dV8xXFxvdmVybGluZXt2fV8xLHVfMlxcb3ZlcmxpbmV7dn1fMn0iXSxbMCwyLCJSIl0sWzEsMSwiUF97dV8xXFxvdmVybGluZXt2fV8xLHVfMnZfMV4qfSJdLFsxLDMsIlBfe3VfMnZfMV4qLHVfMlxcb3ZlcmxpbmV7dn1fMn0iXSxbMiwyLCJEXioiXSxbMiwwLCJEIl0sWzIsNCwiRCciXSxbNCwyLCJCJyJdLFszLDMsIlBfe3ZfMSx2XzJ9Il0sWzQsNCwiQicnIl0sWzUsMywiQyJdLFswLDQsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzEsMCwiciIsMl0sWzEsMiwiXFxwaV8xIl0sWzEsMywiXFxwaV8yIiwyXSxbMiw0LCJcXHBpJ197RF4qfSJdLFszLDQsIlxccGknJ197RF4qfSIsMl0sWzIsNSwiXFxwaSdfRCJdLFszLDYsIlxccGknJ197RCd9IiwyXSxbNCw3LCJmXzJeKiJdLFs1LDcsIlxcb3ZlcmxpbmV7Zn1fMSJdLFszLDgsInhfe3ZfMSx2XzJ9IiwxXSxbOCw3LCJcXHBpX3tCJ30iLDFdLFs4LDksIlxccGlfe0InJ30iLDFdLFs2LDksIlxcb3ZlcmxpbmV7Zn1fMiIsMl0sWzcsMTAsImdfMSJdLFs5LDEwLCJnXzIiLDJdLFswLDUsIlxccGlfRCJdLFsxLDExLCJyIiwyXSxbMTEsNiwiXFxwaV97RCd9IiwyXSxbMTMsMTQsIlxccmhvIiwwLHsib2Zmc2V0IjotNSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxOSwyMiwiIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjQwLCJ0YXJnZXQiOjMwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyMywyNCwiIiwxLHsib2Zmc2V0Ijo1LCJzaG9ydGVuIjp7InNvdXJjZSI6NDAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIyLDIzLCJcXGdhbW1hIiwwLHsib2Zmc2V0IjotNSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsyMCwxOSwiXFx0aWxkZVxcYmV0YSIsMix7Im9mZnNldCI6NSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxMiwxNywiIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjMwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyOCwxOCwiIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\begin{equation}\begin{tikzcd}[ampersand replacement=\&]\label{initial_diagram}
	{P_{u_1\overline{v}_1,u_2\overline{v}_2}} \&\& D \\
	\& {P_{u_1\overline{v}_1,u_2v_1^*}} \\
	R \&\& {D^*} \&\& {B'} \\
	\& {P_{u_2v_1^*,u_2\overline{v}_2}} \&\& {P_{v_1,v_2}} \&\& C \\
	{P_{u_1\overline{v}_1,u_2\overline{v}_2}} \&\& {D'} \&\& {B''}
	\arrow[""{name=0, anchor=center, inner sep=0}, "r"', from=3-1, to=1-1]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi_1}", from=3-1, to=2-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\pi_2}"', from=3-1, to=4-2]
	\arrow["{\pi'_{D^*}}", from=2-2, to=3-3]
	\arrow["{\pi''_{D^*}}"', from=4-2, to=3-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\pi'_D}", from=2-2, to=1-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\pi''_{D'}}"', from=4-2, to=5-3]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{f_2^*}", from=3-3, to=3-5]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\overline{f}_1}", from=1-3, to=3-5]
	\arrow["{x_{v_1,v_2}}"{description}, from=4-2, to=4-4]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{\pi_{B'}}"{description}, from=4-4, to=3-5]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{\pi_{B''}}"{description}, from=4-4, to=5-5]
	\arrow[""{name=9, anchor=center, inner sep=0}, "{\overline{f}_2}"', from=5-3, to=5-5]
	\arrow["{g_1}", from=3-5, to=4-6]
	\arrow["{g_2}"', from=5-5, to=4-6]
	\arrow["{\pi_D}", from=1-1, to=1-3]
	\arrow[""{name=10, anchor=center, inner sep=0}, "r"', from=3-1, to=5-1]
	\arrow["{\pi_{D'}}"', from=5-1, to=5-3]
	\arrow["\rho", shift left=5, shorten <=4pt, shorten >=4pt, Rightarrow, from=1, to=2]
	\arrow[shorten <=7pt, shorten >=5pt, Rightarrow, no head, from=5, to=7]
	\arrow[shift right=5, shorten <=7pt, shorten >=4pt, Rightarrow, no head, from=8, to=9]
	\arrow["\gamma", shift left=5, shorten <=4pt, shorten >=4pt, Rightarrow, from=7, to=8]
	\arrow["\tilde\beta"', shift right=5, shorten <=4pt, shorten >=4pt, Rightarrow, from=6, to=5]
	\arrow[shorten <=19pt, shorten >=19pt, Rightarrow, no head, from=0, to=3]
	\arrow[shorten <=13pt, shorten >=13pt, Rightarrow, no head, from=10, to=4]
\end{tikzcd}\end{equation}

We need to show that the 2-cell diagram that we constructed in Section  \ref{horcomppb} 
$$\xymatrix@C=5em{
&&D\ar[dll]_{u_1\overline{v}_1}\ar[r]^{\overline{f}_1} & B'\ar[dr]^{g_1}
\\
A\ar@{}[rr]|{\rho_{u_1\overline{v}_1,u_2\overline{v}_2}\Downarrow} && P_{u_1\overline{v}_1,u_2\overline{v}_2}\ar@{}[ur]|=\ar@{}[dr]|=\ar[u]_{\pi_{D}}\ar[d]^{\pi_{D'}} \ar[r]^{w_{v_1,v_2}} & P_{v_1,v_2}\ar[u]_{\pi_{B'}}\ar[d]^{\pi_{B''}}\ar@{}[r]|{\gamma\Downarrow} & C\\
&&D'\ar[ull]^{u_2\overline{v}_2}\ar[r]_{\overline{f}_2} & B''\ar[ur]_{g_2}
}
$$
is equvialent to the following diagram, whose right side is the lift of \ref{initial_diagram} with respect to $r$:  
$$
\xymatrix@C=5em{&&D\ar[dll]_{u_1\overline{v}_1}\ar[drr]^{g_1\overline{f}_1} &&
\\
A\ar@{}[rr]|{\rho_{u_1\overline{v}_1,u_2\overline{v}_2}\Downarrow} &&
P_{u_1\overline{v}_1,u_2\overline{v}_2}\ar[u]_{\pi_{D}}\ar[d]^{\pi_{D'}}\ar@{}[rr]|{\widetilde{\beta\gamma}}&& C
\\
&&D'\ar[ull]^{u_2\overline{v}_2}\ar[urr]_{g_2\overline{f}_2} &&
}
$$


To do this, we precompose by $r$, which , which allows us to expand $\widetilde{\beta\gamma}$, replacing it with (\ref{initial_diagram}).
Let diagram (\ref{diagram_A}) be the following sub-diagram of the result:  
\begin{equation}\label{diagram_A} \tag{\bf I}
% https://q.uiver.app/?q=WzAsOCxbMCwxLCJSIl0sWzIsMCwiUF97dV8xXFxvdmVybGluZXt2fV8xLHVfMlxcb3ZlcmxpbmV7dn1fMn0iXSxbMiwxLCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsdV8ydl8xXip9Il0sWzIsMiwiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFs0LDAsIkQiXSxbNCwxLCJEXioiXSxbNiwxLCJCJyJdLFs0LDIsIlBfe3ZfMSx2XzJ9Il0sWzAsMiwiXFxwaV8xIiwyXSxbMCwxLCJyIl0sWzAsMywiXFxwaV8yIiwyXSxbMiw1LCJcXHBpJ197RF4qfSIsMV0sWzMsNSwiXFxwaScnX3tEXip9IiwyXSxbMSw0LCJcXHBpX0QiXSxbMiw0LCJcXHBpX3tEJ30iLDFdLFs0LDYsIlxcb3ZlcmxpbmV7Zn1fMSJdLFs1LDYsImZfMl4qIiwxXSxbMyw3LCJ4X3t2XzEsdl8yfSIsMl0sWzcsNiwiXFxwaV97Qid9IiwxXSxbMTMsMTQsIiIsMCx7Im9mZnNldCI6NSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMSwxMiwiXFxyaG8iLDIseyJvZmZzZXQiOjUsInNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XSxbMTUsMTYsIlxcdGlsZGVcXGJldGEiLDIseyJvZmZzZXQiOjUsInNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XSxbMTYsMTgsIiIsMix7Im9mZnNldCI6NSwic2hvcnRlbiI6eyJzb3VyY2UiOjUwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\begin{tikzcd}[ampersand replacement=\&]
	\&\& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \&\& D \\
	R \&\& {P_{u_1\overline{v}_1,u_2v_1^*}} \&\& {D^*} \&\& {B'} \\
	\&\& {P_{u_2v_1^*,u_2\overline{v}_2}} \&\& {P_{v_1,v_2}}
	\arrow["{\pi_1}"', from=2-1, to=2-3]
	\arrow["r", from=2-1, to=1-3]
	\arrow["{\pi_2}"', from=2-1, to=3-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi'_{D^*}}"{description}, from=2-3, to=2-5]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi''_{D^*}}"', from=3-3, to=2-5]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\pi_D}", from=1-3, to=1-5]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\pi_{D'}}"{description}, from=2-3, to=1-5]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\overline{f}_1}", from=1-5, to=2-7]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{f_2^*}"{description}, from=2-5, to=2-7]
	\arrow["{x_{v_1,v_2}}"', from=3-3, to=3-5]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\pi_{B'}}"{description}, from=3-5, to=2-7]
	\arrow[shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, no head, from=2, to=3]
	\arrow["\rho"', shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, from=0, to=1]
	\arrow["\tilde\beta"', shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, from=4, to=5]
	\arrow[shift right=5, shorten <=5pt, Rightarrow, no head, from=5, to=6]
\end{tikzcd}
\end{equation}
So diagram  (\ref{initial_diagram}) is obtained from  diagram (\ref{diagram_A}) by postcomposing it with $g_1$ and then with $\gamma$. 
We now take diagram (\ref{diagram_A}) and postcompose with $v_1$. 
% https://q.uiver.app/?q=WzAsOSxbMCwxLCJSIl0sWzIsMCwiUF97dV8xXFxvdmVybGluZXt2fV8xLHVfMlxcb3ZlcmxpbmV7dn1fMn0iXSxbMiwxLCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsdV8ydl8xXip9Il0sWzIsMiwiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFs0LDAsIkQiXSxbNCwxLCJEXioiXSxbNiwxLCJCJyJdLFs0LDIsIlBfe3ZfMSx2XzJ9Il0sWzcsMSwiQiJdLFswLDIsIlxccGlfMSIsMl0sWzAsMSwiciJdLFswLDMsIlxccGlfMiIsMl0sWzIsNSwiXFxwaSdfe0ReKn0iLDFdLFszLDUsIlxccGknJ197RF4qfSIsMl0sWzEsNCwiXFxwaV9EIl0sWzIsNCwiXFxwaV97RCd9IiwxXSxbNCw2LCJcXG92ZXJsaW5le2Z9XzEiXSxbNSw2LCJmXzJeKiIsMV0sWzMsNywieF97dl8xLHZfMn0iLDJdLFs3LDYsIlxccGlfe0InfSIsMV0sWzYsOCwidl8xIl0sWzE0LDE1LCIiLDAseyJvZmZzZXQiOjUsInNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTIsMTMsIlxccmhvIiwyLHsib2Zmc2V0Ijo1LCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzE2LDE3LCJcXHRpbGRlXFxiZXRhIiwyLHsib2Zmc2V0Ijo1LCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzE3LDE5LCIiLDIseyJvZmZzZXQiOjUsInNob3J0ZW4iOnsic291cmNlIjo1MH0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
\[\begin{tikzcd}[ampersand replacement=\&]
	\&\& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \&\& D \\
	R \&\& {P_{u_1\overline{v}_1,u_2v_1^*}} \&\& {D^*} \&\& {B'} \& B \\
	\&\& {P_{u_2v_1^*,u_2\overline{v}_2}} \&\& {P_{v_1,v_2}}
	\arrow["{\pi_1}"', from=2-1, to=2-3]
	\arrow["r", from=2-1, to=1-3]
	\arrow["{\pi_2}"', from=2-1, to=3-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi'_{D^*}}"{description}, from=2-3, to=2-5]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi''_{D^*}}"', from=3-3, to=2-5]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\pi_D}", from=1-3, to=1-5]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\pi_{D'}}"{description}, from=2-3, to=1-5]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\overline{f}_1}", from=1-5, to=2-7]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{f_2^*}"{description}, from=2-5, to=2-7]
	\arrow["{x_{v_1,v_2}}"', from=3-3, to=3-5]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\pi_{B'}}"{description}, from=3-5, to=2-7]
	\arrow["{v_1}", from=2-7, to=2-8]
	\arrow[shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, no head, from=2, to=3]
	\arrow["\rho"', shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, from=0, to=1]
	\arrow["\tilde\beta"', shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, from=4, to=5]
	\arrow[shift right=5, shorten <=5pt, Rightarrow, no head, from=5, to=6]
\end{tikzcd}\]
Since $\tilde{\beta}$ was originally defined as a lift with respect to $v_1$, this  allows us to expand $\tilde\beta$:
% https://q.uiver.app/?q=WzAsMTIsWzAsMiwiUiJdLFswLDAsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzAsNCwiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFsxLDIsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJ2XzFeKn0iXSxbMSwwLCJEIl0sWzEsNCwiRF4qIl0sWzIsMSwiQSciXSxbMiwyLCJQX3t1XzEsdV8yfSJdLFsyLDMsIkEnJyJdLFs0LDIsIkIiXSxbMywwLCJCJyJdLFszLDQsIkInIl0sWzAsMSwiciJdLFswLDIsIlxccGlfMiIsMl0sWzAsMywiXFxwaV8xIiwyXSxbMiw1LCJcXHBpJydfe0ReKn0iLDJdLFszLDUsIlxccGknX3tEXip9IiwxXSxbMyw0LCJcXHBpJ19EIiwxXSxbMSw0LCJcXHBpX0QiXSxbNCw2LCJcXG92ZXJsaW5le3Z9XzEiLDFdLFs2LDksImZfMSIsMV0sWzgsOSwiZl8yIiwxXSxbNyw2LCJcXHBpX3tBJ30iLDJdLFs3LDgsIlxccGlfe0EnJ30iXSxbNCwxMCwiXFxvdmVybGluZXtmfV8xIl0sWzEwLDksInZfMSJdLFszLDcsIndeKl97dV8xLHVfMn0iLDJdLFs1LDgsInZfMV4qIiwxXSxbNSwxMSwiZl8yXioiLDJdLFsxMSw5LCJ2XzEiLDJdLFsxNCwxNSwiXFxyaG8iLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6NDAsInRhcmdldCI6MzB9fV0sWzE4LDE0LCIiLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6MzAsInRhcmdldCI6MzB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIwLDIxLCJcXGJldGEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzI0LDIwLCJcXGRlbHRhXzEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MzAsInRhcmdldCI6MzB9fV0sWzE5LDI2LCIiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MzAsInRhcmdldCI6MzB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzI3LDI2LCIiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6NDB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIxLDI4LCJcXHZhcmVwc2lsb25fezEsMn0iLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MzAsInRhcmdldCI6MzB9fV1d
\[\begin{tikzcd}[ampersand replacement=\&]
	{P_{u_1\overline{v}_1,u_2\overline{v}_2}} \& D \&\& {B'} \\
	\&\& {A'} \\
	R \& {P_{u_1\overline{v}_1,u_2v_1^*}} \& {P_{u_1,u_2}} \&\& B \\
	\&\& {A''} \\
	{P_{u_2v_1^*,u_2\overline{v}_2}} \& {D^*} \&\& {B'}
	\arrow["r", from=3-1, to=1-1]
	\arrow["{\pi_2}"', from=3-1, to=5-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi_1}"', from=3-1, to=3-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi''_{D^*}}"', from=5-1, to=5-2]
	\arrow["{\pi'_{D^*}}"{description}, from=3-2, to=5-2]
	\arrow["{\pi'_D}"{description}, from=3-2, to=1-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\pi_D}", from=1-1, to=1-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\overline{v}_1}"{description}, from=1-2, to=2-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{f_1}"{description}, from=2-3, to=3-5]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{f_2}"{description}, from=4-3, to=3-5]
	\arrow["{\pi_{A'}}"', from=3-3, to=2-3]
	\arrow["{\pi_{A''}}", from=3-3, to=4-3]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\overline{f}_1}", from=1-2, to=1-4]
	\arrow["{v_1}", from=1-4, to=3-5]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{w^*_{u_1,u_2}}"', from=3-2, to=3-3]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{v_1^*}"{description}, from=5-2, to=4-3]
	\arrow[""{name=9, anchor=center, inner sep=0}, "{f_2^*}"', from=5-2, to=5-4]
	\arrow["{v_1}"', from=5-4, to=3-5]
	\arrow["\rho"', shorten <=17pt, shorten >=13pt, Rightarrow, from=0, to=1]
	\arrow[shorten <=13pt, shorten >=13pt, Rightarrow, no head, from=2, to=0]
	\arrow["\beta"{description}, shorten <=4pt, shorten >=4pt, Rightarrow, from=4, to=5]
	\arrow["{\delta_1}"{description}, shorten <=13pt, shorten >=13pt, Rightarrow, from=6, to=4]
	\arrow[shorten <=10pt, shorten >=10pt, Rightarrow, no head, from=3, to=7]
	\arrow[shorten <=6pt, shorten >=13pt, Rightarrow, no head, from=8, to=7]
	\arrow["{\varepsilon_{1,2}^{-1}}"{description}, shorten <=13pt, shorten >=13pt, Rightarrow, from=5, to=9]
\end{tikzcd}\]
We now postcompose by $\rho_{v_1,v_2}$.
% https://q.uiver.app/?q=WzAsMTUsWzAsMiwiUiJdLFswLDAsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzAsNSwiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFsxLDIsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJ2XzFeKn0iXSxbMSwwLCJEIl0sWzEsNCwiRF4qIl0sWzIsMSwiQSciXSxbMiwyLCJQX3t1XzEsdV8yfSJdLFsyLDMsIkEnJyJdLFs1LDQsIkIiXSxbNSwyLCJCJyJdLFszLDQsIkInIl0sWzEsNSwiUF97dl8xLHZfMn0iXSxbMyw1LCJCJyciXSxbMSw2LCJEJyJdLFswLDEsInIiXSxbMCwyLCJcXHBpXzIiLDJdLFswLDMsIlxccGlfMSIsMl0sWzIsNSwiXFxwaScnX3tEXip9IiwyXSxbMyw1LCJcXHBpJ197RF4qfSIsMV0sWzMsNCwiXFxwaSdfRCIsMV0sWzEsNCwiXFxwaV9EIl0sWzQsNiwiXFxvdmVybGluZXt2fV8xIiwxXSxbNiw5LCJmXzEiLDFdLFs4LDksImZfMiIsMV0sWzcsNiwiXFxwaV97QSd9IiwyXSxbNyw4LCJcXHBpX3tBJyd9Il0sWzQsMTAsIlxcb3ZlcmxpbmV7Zn1fMSJdLFsxMCw5LCJ2XzEiXSxbMyw3LCJ3Xipfe3VfMSx1XzJ9IiwyXSxbNSw4LCJ2XzFeKiIsMV0sWzUsMTEsImZfMl4qIiwxXSxbMTEsOSwidl8xIiwxXSxbMiwxMiwieF97dl8xLHZfMn0iLDJdLFsxMiwxMSwiXFxwaV97Qid9IiwxXSxbMTIsMTMsIlxccGlfe0InJ30iLDFdLFsxMyw5LCJ2XzIiLDJdLFsyLDE0LCJcXHBpJydfe0QnfSIsMl0sWzE0LDEzLCJcXG92ZXJsaW5le2Z9XzIiLDJdLFsxNywxOCwiXFxyaG8iLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6NDAsInRhcmdldCI6MzB9fV0sWzIxLDE3LCIiLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6MzAsInRhcmdldCI6MzB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIzLDI0LCJcXGJldGEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzI3LDIzLCJcXGRlbHRhXzEiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MzAsInRhcmdldCI6MzB9fV0sWzIyLDI5LCIiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MzAsInRhcmdldCI6MzB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMwLDI5LCIiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6NDB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMxLDM0LCIiLDEseyJvZmZzZXQiOjUsInNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMzIsMzYsIlxccmhvX3t2XzEsdl8yfSIsMix7Im9mZnNldCI6NSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFszMCwzMSwiXFx2YXJlcHNpbG9uX3sxLDJ9IiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjMwfX1dLFszNSwzOCwiIiwxLHsib2Zmc2V0Ijo1LCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}[ampersand replacement=\&]
	{P_{u_1\overline{v}_1,u_2\overline{v}_2}} \& D \\
	\&\& {A'} \\
	R \& {P_{u_1\overline{v}_1,u_2v_1^*}} \& {P_{u_1,u_2}} \&\&\& {B'} \\
	\&\& {A''} \\
	\& {D^*} \&\& {B'} \&\& B \\
	{P_{u_2v_1^*,u_2\overline{v}_2}} \& {P_{v_1,v_2}} \&\& {B''} \\
	\& {D'}
	\arrow["r", from=3-1, to=1-1]
	\arrow["{\pi_2}"', from=3-1, to=6-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi_1}"', from=3-1, to=3-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi''_{D^*}}"', from=6-1, to=5-2]
	\arrow["{\pi'_{D^*}}"{description}, from=3-2, to=5-2]
	\arrow["{\pi'_D}"{description}, from=3-2, to=1-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\pi_D}", from=1-1, to=1-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\overline{v}_1}"{description}, from=1-2, to=2-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{f_1}"{description}, from=2-3, to=5-6]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{f_2}"{description}, from=4-3, to=5-6]
	\arrow["{\pi_{A'}}"', from=3-3, to=2-3]
	\arrow["{\pi_{A''}}", from=3-3, to=4-3]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\overline{f}_1}", from=1-2, to=3-6]
	\arrow["{v_1}", from=3-6, to=5-6]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{w^*_{u_1,u_2}}"', from=3-2, to=3-3]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{v_1^*}"{description}, from=5-2, to=4-3]
	\arrow[""{name=9, anchor=center, inner sep=0}, "{f_2^*}"{description}, from=5-2, to=5-4]
	\arrow[""{name=10, anchor=center, inner sep=0}, "{v_1}"{description}, from=5-4, to=5-6]
	\arrow["{x_{v_1,v_2}}"', from=6-1, to=6-2]
	\arrow[""{name=11, anchor=center, inner sep=0}, "{\pi_{B'}}"{description}, from=6-2, to=5-4]
	\arrow[""{name=12, anchor=center, inner sep=0}, "{\pi_{B''}}"{description}, from=6-2, to=6-4]
	\arrow[""{name=13, anchor=center, inner sep=0}, "{v_2}"', from=6-4, to=5-6]
	\arrow["{\pi''_{D'}}"', from=6-1, to=7-2]
	\arrow[""{name=14, anchor=center, inner sep=0}, "{\overline{f}_2}"', from=7-2, to=6-4]
	\arrow["\rho"', shorten <=21pt, shorten >=16pt, Rightarrow, from=0, to=1]
	\arrow[shorten <=13pt, shorten >=13pt, Rightarrow, no head, from=2, to=0]
	\arrow["\beta"{description}, shorten <=4pt, shorten >=4pt, Rightarrow, from=4, to=5]
	\arrow["{\delta_1}"{description}, shorten <=11pt, shorten >=11pt, Rightarrow, from=6, to=4]
	\arrow[shorten <=10pt, shorten >=10pt, Rightarrow, no head, from=3, to=7]
	\arrow[shorten <=6pt, shorten >=13pt, Rightarrow, no head, from=8, to=7]
	\arrow[shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, no head, from=9, to=11]
	\arrow["{\rho_{v_1,v_2}}"', shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, from=10, to=13]
	\arrow["{\varepsilon_{1,2}^{-1}}", shorten <=5pt, shorten >=5pt, Rightarrow, from=8, to=9]
	\arrow[shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, no head, from=12, to=14]
\end{tikzcd}\]
By the definition of $x_{v_1,v_2}$ this is equal to
% https://q.uiver.app/?q=WzAsMTUsWzYsMiwiQiJdLFs1LDAsIkInIl0sWzQsMSwiQSciXSxbNCwyLCJBJyciXSxbNSwzLCJCJyJdLFs1LDQsIkEnJyJdLFs2LDQsIkInJyJdLFszLDAsIkQiXSxbMywyLCJQX3t1XzEsdV8yfSJdLFsxLDIsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJ2XzFeKn0iXSxbMSwxLCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsdV8yXFxvdmVybGluZXt2fV8yfSJdLFswLDMsIlIiXSxbMywzLCJEXioiXSxbNSw1LCJEJyJdLFsxLDQsIlBfe3VfMnZfMV4qLHVfMlxcb3ZlcmxpbmV7dn1fMn0iXSxbMSwwLCJ2XzEiXSxbMiwwLCJmXzEiLDFdLFszLDAsImZfMiIsMV0sWzQsMCwidl8xIiwxXSxbNSwwLCJmXzIiLDFdLFs2LDAsInZfMiIsMV0sWzcsMiwiXFxvdmVybGluZXt2fV8xIiwyXSxbNywxLCJcXG92ZXJsaW5le2Z9XzEiXSxbOCwyLCJcXHBpX3tBJ30iLDFdLFs4LDMsIlxccGlfe0EnJ30iLDJdLFs5LDgsIndeKl97dV8xLHVfMn0iLDFdLFs5LDcsIlxccGlfRCciLDFdLFsxMCw3LCJcXHBpX0QiXSxbMTEsMTAsInIiXSxbMTEsOSwiXFxwaV8xIiwxXSxbMTIsNCwiZl8yXioiLDFdLFsxMiwzLCJ2XzFeKiIsMV0sWzEyLDUsInZfMV4qIiwxXSxbMTMsNiwiXFxvdmVybGluZXtmfV8yIiwyXSxbMTMsNSwiXFxvdmVybGluZXt2fV8yIiwyXSxbMTQsMTIsIlxccGknJ197RF4qfSIsMV0sWzE0LDEzLCJcXHBpJydfe0QnfSIsMl0sWzksMTIsIlxccGknX3tEXip9IiwyXSxbMTEsMTQsIlxccGlfMiIsMl0sWzIyLDE2LCJcXGRlbHRhXzEiLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzE2LDE3LCJcXGJldGEiLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzI2LDIzLCIiLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MzB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzI4LDI2LCIiLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE3LDMwLCJcXHZhcmVwc2lsb25fezEsMn1eey0xfSIsMix7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XSxbMTksMzMsIlxcZGVsdGFfMl57LTF9IiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjQwLCJ0YXJnZXQiOjMwfX1dLFsyNSwzNywiIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszNywzOCwiXFxyaG8iLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzMwLDMyLCJcXHZhcmVwc2lsb25fezEsMn0iLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzMyLDM2LCJcXHRpbGRle1xccmhvfV97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSIsMCx7Im9mZnNldCI6NSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dXQ==
\[\begin{tikzcd}[ampersand replacement=\&]
	\&\&\& D \&\& {B'} \\
	\& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \&\&\& {A'} \\
	\& {P_{u_1\overline{v}_1,u_2v_1^*}} \&\& {P_{u_1,u_2}} \& {A''} \&\& B \\
	R \&\&\& {D^*} \&\& {B'} \\
	\& {P_{u_2v_1^*,u_2\overline{v}_2}} \&\&\&\& {A''} \& {B''} \\
	\&\&\&\&\& {D'}
	\arrow["{v_1}", from=1-6, to=3-7]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{f_1}"{description}, from=2-5, to=3-7]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{f_2}"{description}, from=3-5, to=3-7]
	\arrow["{v_1}"{description}, from=4-6, to=3-7]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{f_2}"{description}, from=5-6, to=3-7]
	\arrow["{v_2}"{description}, from=5-7, to=3-7]
	\arrow["{\overline{v}_1}"', from=1-4, to=2-5]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\overline{f}_1}", from=1-4, to=1-6]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\pi_{A'}}"{description}, from=3-4, to=2-5]
	\arrow["{\pi_{A''}}"', from=3-4, to=3-5]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{w^*_{u_1,u_2}}"{description}, from=3-2, to=3-4]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\pi_D'}"{description}, from=3-2, to=1-4]
	\arrow["{\pi_D}", from=2-2, to=1-4]
	\arrow[""{name=7, anchor=center, inner sep=0}, "r", from=4-1, to=2-2]
	\arrow["{\pi_1}"{description}, from=4-1, to=3-2]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{f_2^*}"{description}, from=4-4, to=4-6]
	\arrow["{v_1^*}"{description}, from=4-4, to=3-5]
	\arrow[""{name=9, anchor=center, inner sep=0}, "{v_1^*}"{description}, from=4-4, to=5-6]
	\arrow[""{name=10, anchor=center, inner sep=0}, "{\overline{f}_2}"', from=6-6, to=5-7]
	\arrow["{\overline{v}_2}"', from=6-6, to=5-6]
	\arrow["{\pi''_{D^*}}"{description}, from=5-2, to=4-4]
	\arrow[""{name=11, anchor=center, inner sep=0}, "{\pi''_{D'}}"', from=5-2, to=6-6]
	\arrow[""{name=12, anchor=center, inner sep=0}, "{\pi'_{D^*}}"', from=3-2, to=4-4]
	\arrow[""{name=13, anchor=center, inner sep=0}, "{\pi_2}"', from=4-1, to=5-2]
	\arrow["{\delta_1}", shorten <=9pt, shorten >=9pt, Rightarrow, from=3, to=0]
	\arrow["\beta", shorten <=2pt, shorten >=2pt, Rightarrow, from=0, to=1]
	\arrow[shorten <=10pt, shorten >=15pt, Rightarrow, no head, from=6, to=4]
	\arrow[shorten <=11pt, shorten >=11pt, Rightarrow, no head, from=7, to=6]
	\arrow["{\varepsilon_{1,2}^{-1}}"', shorten <=7pt, shorten >=7pt, Rightarrow, from=1, to=8]
	\arrow["{\delta_2^{-1}}", shorten <=13pt, shorten >=10pt, Rightarrow, from=2, to=10]
	\arrow[shorten <=2pt, shorten >=2pt, Rightarrow, no head, from=5, to=12]
	\arrow["\rho"{description}, shorten <=12pt, shorten >=12pt, Rightarrow, from=12, to=13]
	\arrow["{\varepsilon_{1,2}}", shorten <=2pt, shorten >=2pt, Rightarrow, from=8, to=9]
	\arrow["{\tilde{\rho}_{u_2v_1^*,u_2\overline{v}_2}}", shift right=5, shorten <=7pt, shorten >=7pt, Rightarrow, from=9, to=11]
\end{tikzcd}\]
We can now cancel $\varepsilon_{1,2}^{-1}$ and $\varepsilon_{1,2}$:
% https://q.uiver.app/?q=WzAsMTMsWzAsMSwiUiJdLFsyLDEsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzQsMSwiUF97dV8xLHVfMn0iXSxbNiwyLCJBJyciXSxbOCwxLCJCIl0sWzYsMSwiQSciXSxbNCwwLCJEIl0sWzYsMCwiQiciXSxbMSwwLCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsdV8yXFxvdmVybGluZXt2fV8yfSJdLFsxLDIsIlBfe3VfMnZfMV4qLHVfMlxcb3ZlcmxpbmV7dn1fMn0iXSxbMywyLCJEXioiXSxbMiwzLCJEJyJdLFs2LDMsIkInJyJdLFsyLDUsIlxccGlfe0EnfSIsMV0sWzIsMywiXFxwaV97QScnfSIsMV0sWzEsMiwid14qX3t1XzEsdV8yfSIsMl0sWzAsMSwiXFxwaV8xIiwyXSxbMSw2LCJcXHBpJ19EIiwxXSxbNiw1LCJcXG92ZXJsaW5le3Z9XzEiXSxbNiw3LCJcXG92ZXJsaW5le2Z9XzEiXSxbOCw2LCJcXHBpX0QiXSxbMCw4LCJyIl0sWzcsNCwidl8xIl0sWzUsNCwiZl8xIiwxXSxbMyw0LCJmXzIiLDFdLFswLDksIlxccGlfMiIsMl0sWzksMTAsIlxccGknJ197RF4qfSIsMl0sWzEsMTAsIlxccGknX3tEXip9IiwxXSxbMTAsMywidl8xXioiLDFdLFs5LDExLCJcXHBpJydfe0QnfSIsMl0sWzExLDMsIlxcb3ZlcmxpbmV7dn1fMiIsMV0sWzExLDEyLCJcXG92ZXJsaW5le2Z9XzIiLDJdLFsxMiw0LCJ2XzIiLDJdLFsyMCwxNiwiIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxOSwyMywiXFxkZWx0YV8xIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxOCwxMywiIiwyLHsib2Zmc2V0Ijo1LCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE0LDI3LCIiLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzI3LDI1LCJcXHJobyIsMCx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XSxbMjYsMzAsIlxcdGlsZGVcXHJob197dV8ydl4qXzEsdV8yXFxvdmVybGluZXt2fV8yfSIsMix7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XSxbMzAsMzEsIlxcZGVsdGFfMl57LTF9IiwwLHsib2Zmc2V0IjotNSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsyMywxNCwiXFxiZXRhIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dXQ==
\begin{equation}\label{number7}
\begin{tikzcd}[ampersand replacement=\&,column sep = small]
	\& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \&\&\& D \&\& {B'} \\
	R \&\& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \&\& {P_{u_1,u_2}} \&\& {A'} \&\& B \\
	\& {P_{u_2v_1^*,u_2\overline{v}_2}} \&\& {D^*} \&\&\& {A''} \\
	\&\& {D'} \&\&\&\& {B''}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi_{A'}}"{description}, from=2-5, to=2-7]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi_{A''}}"{description}, from=2-5, to=3-7]
	\arrow["{w^*_{u_1,u_2}}"', from=2-3, to=2-5]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\pi_1}"', from=2-1, to=2-3]
	\arrow["{\pi'_D}"{description}, from=2-3, to=1-5]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\overline{v}_1}", from=1-5, to=2-7]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\overline{f}_1}", from=1-5, to=1-7]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{\pi_D}", from=1-2, to=1-5]
	\arrow["r", from=2-1, to=1-2]
	\arrow["{v_1}", from=1-7, to=2-9]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{f_1}"{description}, from=2-7, to=2-9]
	\arrow["{f_2}"{description}, from=3-7, to=2-9]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{\pi_2}"', from=2-1, to=3-2]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{\pi''_{D^*}}"', from=3-2, to=3-4]
	\arrow[""{name=9, anchor=center, inner sep=0}, "{\pi'_{D^*}}"{description}, from=2-3, to=3-4]
	\arrow["{v_1^*}"{description}, from=3-4, to=3-7]
	\arrow["{\pi''_{D'}}"', from=3-2, to=4-3]
	\arrow[""{name=10, anchor=center, inner sep=0}, "{\overline{v}_2}"{description}, from=4-3, to=3-7]
	\arrow[""{name=11, anchor=center, inner sep=0}, "{\overline{f}_2}"', from=4-3, to=4-7]
	\arrow["{v_2}"', from=4-7, to=2-9]
	\arrow[shorten <=13pt, shorten >=13pt, Rightarrow, no head, from=5, to=2]
	\arrow["{\delta_1}", shorten <=13pt, shorten >=13pt, Rightarrow, from=4, to=6]
	\arrow[shift right=5, shorten <=2pt, shorten >=2pt, Rightarrow, no head, from=3, to=0]
	\arrow[shorten <=17pt, shorten >=17pt, Rightarrow, no head, from=1, to=9]
	\arrow["\rho", shorten <=17pt, shorten >=17pt, Rightarrow, from=9, to=7]
	\arrow["{\tilde\rho_{u_2v^*_1,u_2\overline{v}_2}}"', shorten <=13pt, shorten >=13pt, Rightarrow, from=8, to=10]
	\arrow["{\delta_2^{-1}}", shift left=5, shorten <=2pt, shorten >=2pt, Rightarrow, from=10, to=11]
	\arrow["\beta", shorten <=13pt, shorten >=13pt, Rightarrow, from=6, to=1]
\end{tikzcd}\end{equation}
We again decide to focus on just a part of this diagram -- we call this part $B$.
% https://q.uiver.app/?q=WzAsOSxbMCwxLCJCIl0sWzEsMSwiXFxlcXVpdiJdLFsyLDEsIlIiXSxbMywwLCJQX3t1X3FcXG92ZXJsaW5le3Z9XzEsdV8ydl8xXip9Il0sWzMsMiwiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFs0LDEsIkReKiJdLFs2LDEsIkEnJyJdLFs1LDAsIlBfe3VfMSx1XzJ9Il0sWzUsMiwiRCciXSxbMiwzLCJcXHBpXzEiXSxbMiw0LCJcXHBpXzIiLDJdLFszLDUsIlxccGlfe0ReKn0nIl0sWzQsNSwiXFxwaScnX3tEXip9IiwyXSxbNSw2LCJ2XzFeKiJdLFszLDcsIndeKl97dV8xLHVfMn0iXSxbNyw2LCJcXHBpX3tBJyd9Il0sWzQsOCwiXFxwaV97RCd9JyciLDJdLFs4LDYsIlxcb3ZlcmxpbmV7dn1fMiIsMl0sWzksMTAsIlxccmhvIiwwLHsib2Zmc2V0IjotNSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxMywxNiwiXFx0aWxkZVxccmhvX3t1XzJ2XzFeKix1XzJcXG92ZXJsaW5le3Z9XzJ9IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxNCwxMywiIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}[ampersand replacement=\&]
	\&\&\& {P_{u_q\overline{v}_1,u_2v_1^*}} \&\& {P_{u_1,u_2}} \\
	{\bf (II)} \& \equiv \& R \&\& {D^*} \&\& {A''} \\
	\&\&\& {P_{u_2v_1^*,u_2\overline{v}_2}} \&\& {D'}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi_1}", from=2-3, to=1-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi_2}"', from=2-3, to=3-4]
	\arrow["{\pi_{D^*}'}", from=1-4, to=2-5]
	\arrow["{\pi''_{D^*}}"', from=3-4, to=2-5]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{v_1^*}", from=2-5, to=2-7]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{w^*_{u_1,u_2}}", from=1-4, to=1-6]
	\arrow["{\pi_{A''}}", from=1-6, to=2-7]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\pi_{D'}''}"', from=3-4, to=3-6]
	\arrow["{\overline{v}_2}"', from=3-6, to=2-7]
	\arrow["\rho", shift left=5, shorten <=4pt, shorten >=4pt, Rightarrow, from=0, to=1]
	\arrow["{\tilde\rho_{u_2v_1^*,u_2\overline{v}_2}}"{description}, shorten <=7pt, shorten >=7pt, Rightarrow, from=2, to=4]
	\arrow[shorten <=7pt, shorten >=7pt, Rightarrow, no head, from=3, to=2]
\end{tikzcd}\]
We will now show that if we post-compose diagram {\bf (II)} with $u_2$, we get   an identity 2-cell. To show this, we post-compose diagram {\bf (II)} with $u_2$ and then pre-compose with the invertible 2-cell $\rho_{u_1,u_2}$:
% https://q.uiver.app/?q=WzAsMjcsWzAsMiwiUiJdLFsxLDEsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzEsMywiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFsyLDIsIkReKiJdLFszLDIsIkEnJyJdLFsyLDEsIlBfe3VfMSx1XzJ9Il0sWzQsMiwiQSJdLFszLDEsIkEnIl0sWzIsMCwiRCJdLFsyLDMsIkQnIl0sWzUsMiwiXFxlcXVpdiJdLFs2LDIsIlIiXSxbNywxLCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsdV8yXFxvdmVybGluZXt2fV8yfSJdLFs3LDMsIlBfe3VfMnZfMV4qLHVfMlxcb3ZlcmxpbmV7dn1fMn0iXSxbOCwyLCJEXioiXSxbOCwwLCJEIl0sWzksMCwiQSciXSxbOSwyLCJBJyciXSxbMTAsMiwiQSJdLFs4LDMsIkQnIl0sWzksMywiQScnIl0sWzUsNSwiXFxlcXVpdiJdLFs2LDUsIlIiXSxbNyw0LCJEIl0sWzcsNiwiRCciXSxbNyw1LCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsdV8yXFxvdmVybGluZXt2fV8yfSJdLFs5LDUsIkEiXSxbMCwyLCJcXHBpXzIiLDJdLFswLDEsIlxccGlfMSJdLFsxLDMsIlxccGknX3tEXip9IiwyXSxbMiwzLCJcXHBpJydfe0ReKn0iXSxbMyw0LCJ2XzFeKiJdLFsxLDUsIndfe3VfMSx1XzJ9XioiXSxbNSw0LCJcXHBpX3tBJyd9IiwxXSxbNCw2LCJ1XzIiXSxbNSw3LCJcXHBpX3tBJ30iXSxbNyw2LCJ1XzEiXSxbMSw4LCJcXHBpJ19EIl0sWzgsNywiXFxvdmVybGluZXt2fV8xIl0sWzksNCwiXFxvdmVybGluZXt2fV8yIiwyXSxbMiw5LCJcXHBpJydfe0QnfSIsMl0sWzExLDEyLCJcXHBpXzEiXSxbMTEsMTMsIlxccGlfMiIsMl0sWzEzLDE0LCJcXHBpJydfe0ReKn0iXSxbMTIsMTQsIlxccGknX3tEXip9IiwyXSxbMTIsMTUsIlxccGknX0QiXSxbMTQsMTcsInZfMV4qIl0sWzE1LDE2LCJcXG92ZXJsaW5le3Z9XzEiXSxbMTcsMTgsInVfMiJdLFsxNiwxOCwidV8xIl0sWzIwLDE4LCJ1XzIiLDJdLFsxOSwyMCwiXFxvdmVybGluZXt2fV8yIiwyXSxbMTMsMTksIlxccGknJ197RCd9IiwyXSxbMjIsMjUsInIiXSxbMjUsMjMsIlxccGlfRCJdLFsyNSwyNCwiXFxwaV97RCd9Il0sWzIyLDI0LCJcXHBpJ197RCd9XFxwaV8yIiwyLHsiY3VydmUiOjF9XSxbMjIsMjMsIlxccGknX0RcXHBpXzEiLDAseyJjdXJ2ZSI6LTF9XSxbMjMsMjYsInVfMVxcb3ZlcmxpbmV7dn1fMSIsMCx7ImN1cnZlIjotMn1dLFsyNCwyNiwidV8yXFxvdmVybGluZXt2fV8yIiwyLHsiY3VydmUiOjJ9XSxbMjgsMjcsIlxccmhvIiwwLHsib2Zmc2V0IjotNSwic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjQwfX1dLFszMiwzMSwiIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjQwLCJ0YXJnZXQiOjMwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszNSwzNCwiXFxyaG9fe3VfMSx1XzJ9IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFszMSw0MCwiXFx0aWxkZVxccmhvX3t1XzJ2XzFeKix1XzJcXG92ZXJsaW5le3Z9XzJ9IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFs0MSw0MiwiXFxyaG8iLDAseyJvZmZzZXQiOi01LCJzaG9ydGVuIjp7InNvdXJjZSI6MzAsInRhcmdldCI6NDB9fV0sWzQ3LDQ2LCJcXHJob197dV8xXFxvdmVybGluZXt2fV8xLHVfMnZfMV4qfSIsMCx7InNob3J0ZW4iOnsic291cmNlIjo0MCwidGFyZ2V0IjozMH19XSxbNDYsNTEsIlxccmhvX3t1XzJ2XzFeKix1XzJcXG92ZXJsaW5le3Z9XzJ9IiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjMwfX1dLFs1Nyw1MywiIiwwLHsib2Zmc2V0IjotNCwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjQwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs1Myw1NiwiIiwwLHsib2Zmc2V0IjotNSwic2hvcnRlbiI6eyJzb3VyY2UiOjQwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs1OCw1OSwiXFxyaG9fe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzIsXFxvdmVybGluZXt2fV8yfSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XSxbMzgsNSwiIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}[ampersand replacement=\&, column sep = small]
	\&\& D \&\&\&\&\&\& D \& {A'} \\
	\& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \& {P_{u_1,u_2}} \& {A'} \&\&\&\& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \\
	R \&\& {D^*} \& {A''} \& A \& \equiv \& R \&\& {D^*} \& {A''} \& A \\
	\& {P_{u_2v_1^*,u_2\overline{v}_2}} \& {D'} \&\&\&\&\& {P_{u_2v_1^*,u_2\overline{v}_2}} \& {D'} \& {A''} \\
	\&\&\&\&\&\&\& D \\
	\&\&\&\&\& \equiv \& R \& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \&\& A \\
	\&\&\&\&\&\&\& {D'}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi_2}"', from=3-1, to=4-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi_1}", from=3-1, to=2-2]
	\arrow["{\pi'_{D^*}}"', from=2-2, to=3-3]
	\arrow["{\pi''_{D^*}}", from=4-2, to=3-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{v_1^*}", from=3-3, to=3-4]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{w_{u_1,u_2}^*}", from=2-2, to=2-3]
	\arrow["{\pi_{A''}}"{description}, from=2-3, to=3-4]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{u_2}", from=3-4, to=3-5]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{\pi_{A'}}", from=2-3, to=2-4]
	\arrow["{u_1}", from=2-4, to=3-5]
	\arrow["{\pi'_D}", from=2-2, to=1-3]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\overline{v}_1}", from=1-3, to=2-4]
	\arrow["{\overline{v}_2}"', from=4-3, to=3-4]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{\pi''_{D'}}"', from=4-2, to=4-3]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{\pi_1}", from=3-7, to=2-8]
	\arrow[""{name=9, anchor=center, inner sep=0}, "{\pi_2}"', from=3-7, to=4-8]
	\arrow["{\pi''_{D^*}}", from=4-8, to=3-9]
	\arrow["{\pi'_{D^*}}"', from=2-8, to=3-9]
	\arrow["{\pi'_D}", from=2-8, to=1-9]
	\arrow[""{name=10, anchor=center, inner sep=0}, "{v_1^*}", from=3-9, to=3-10]
	\arrow[""{name=11, anchor=center, inner sep=0}, "{\overline{v}_1}", from=1-9, to=1-10]
	\arrow["{u_2}", from=3-10, to=3-11]
	\arrow["{u_1}", from=1-10, to=3-11]
	\arrow["{u_2}"', from=4-10, to=3-11]
	\arrow[""{name=12, anchor=center, inner sep=0}, "{\overline{v}_2}"', from=4-9, to=4-10]
	\arrow["{\pi''_{D'}}"', from=4-8, to=4-9]
	\arrow[""{name=13, anchor=center, inner sep=0}, "r", from=6-7, to=6-8]
	\arrow["{\pi_D}", from=6-8, to=5-8]
	\arrow["{\pi_{D'}}", from=6-8, to=7-8]
	\arrow[""{name=14, anchor=center, inner sep=0}, "{\pi'_{D'}\pi_2}"', curve={height=6pt}, from=6-7, to=7-8]
	\arrow[""{name=15, anchor=center, inner sep=0}, "{\pi'_D\pi_1}", curve={height=-6pt}, from=6-7, to=5-8]
	\arrow[""{name=16, anchor=center, inner sep=0}, "{u_1\overline{v}_1}", curve={height=-12pt}, from=5-8, to=6-10]
	\arrow[""{name=17, anchor=center, inner sep=0}, "{u_2\overline{v}_2}"', curve={height=12pt}, from=7-8, to=6-10]
	\arrow["\rho", shift left=5, shorten <=6pt, shorten >=8pt, Rightarrow, from=1, to=0]
	\arrow[shorten <=15pt, shorten >=11pt, Rightarrow, no head, from=3, to=2]
	\arrow["{\rho_{u_1,u_2}}"{description}, shorten <=7pt, shorten >=7pt, Rightarrow, from=5, to=4]
	\arrow["{\tilde\rho_{u_2v_1^*,u_2\overline{v}_2}}"{description}, shorten <=7pt, shorten >=7pt, Rightarrow, from=2, to=7]
	\arrow["\rho", shift left=5, shorten <=6pt, shorten >=8pt, Rightarrow, from=8, to=9]
	\arrow["{\rho_{u_1\overline{v}_1,u_2v_1^*}}", shorten <=17pt, shorten >=13pt, Rightarrow, from=11, to=10]
	\arrow["{\rho_{u_2v_1^*,u_2\overline{v}_2}}", shorten <=6pt, shorten >=6pt, Rightarrow, from=10, to=12]
	\arrow[shift left=4, shorten <=3pt, shorten >=6pt, Rightarrow, no head, from=15, to=13]
	\arrow[shift left=5, shorten <=6pt, shorten >=3pt, Rightarrow, no head, from=13, to=14]
	\arrow["{\rho_{u_1\overline{v}_1,u_2,\overline{v}_2}}"{description}, shorten <=7pt, shorten >=7pt, Rightarrow, from=16, to=17]
	\arrow[shorten <=2pt, Rightarrow, no head, from=6, to=2-3]
\end{tikzcd}\]
The first equality above follows from the universal property of the arrow $w^*_{u_1,u_2}$, and the second equality follows from the definition of the arrow $r$. The definition of $w_{u_1,u_2}$ now implies that this pasting is equal to
% https://q.uiver.app/?q=WzAsMTAsWzAsMSwiUiJdLFswLDAsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJ2XzFeKn0iXSxbMCwyLCJQX3t1XzJ2XzFeKix1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzEsMSwiUF97dV8xLFxcb3ZlcmxpbmV7dn1fMSx1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzEsMCwiRCJdLFsxLDIsIkQnIl0sWzIsMCwiQSciXSxbMiwxLCJQX3t1XzEsdV8yfSJdLFszLDEsIkEnJyJdLFs0LDEsIkEiXSxbOCw5LCJ1XzIiLDFdLFs3LDgsIlxccGlfe0EnJ30iXSxbMyw3LCJ3X3t1XzEsdV8yfSJdLFs3LDYsIlxccGlfe0EnfSIsMl0sWzYsOSwidV8xIiwwLHsiY3VydmUiOi0yfV0sWzUsOCwiXFxvdmVybGluZXt2fV8yIiwyLHsiY3VydmUiOjJ9XSxbMyw1LCJcXHBpX3tEJ30iXSxbMyw0LCJcXHBpX0QiLDJdLFs0LDYsIlxcb3ZlcmxpbmV7dn1fMSJdLFswLDMsInIiLDJdLFswLDEsIlxccGlfMSJdLFswLDIsIlxccGlfMiIsMl0sWzIsNSwiXFxwaScnX3tEJ30iLDJdLFsxLDQsIlxccGknX0QiXSxbMTQsOCwiXFxyaG9fe3VfMSx1XzJ9IiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjMwfX1dLFsxMiwxNSwiIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjQwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxOCwxMiwiIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjQwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxOSwyMiwiIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjQwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyMywxOSwiIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjMwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}[ampersand replacement=\&]
	{P_{u_1\overline{v}_1,u_2v_1^*}} \& D \& {A'} \\
	R \& {P_{u_1,\overline{v}_1,u_2\overline{v}_2}} \& {P_{u_1,u_2}} \& {A''} \& A \\
	{P_{u_2v_1^*,u_2\overline{v}_2}} \& {D'}
	\arrow["{u_2}"{description}, from=2-4, to=2-5]
	\arrow["{\pi_{A''}}", from=2-3, to=2-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{w_{u_1,u_2}}", from=2-2, to=2-3]
	\arrow["{\pi_{A'}}"', from=2-3, to=1-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{u_1}", curve={height=-12pt}, from=1-3, to=2-5]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\overline{v}_2}"', curve={height=12pt}, from=3-2, to=2-4]
	\arrow["{\pi_{D'}}", from=2-2, to=3-2]
	\arrow["{\pi_D}"', from=2-2, to=1-2]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\overline{v}_1}", from=1-2, to=1-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "r"', from=2-1, to=2-2]
	\arrow["{\pi_1}", from=2-1, to=1-1]
	\arrow["{\pi_2}"', from=2-1, to=3-1]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{\pi''_{D'}}"', from=3-1, to=3-2]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\pi'_D}", from=1-1, to=1-2]
	\arrow["{\rho_{u_1,u_2}}"', shorten <=3pt, shorten >=4pt, Rightarrow, from=1, to=2-4]
	\arrow[shorten <=7pt, shorten >=9pt, Rightarrow, no head, from=0, to=2]
	\arrow[shorten <=6pt, shorten >=9pt, Rightarrow, no head, from=3, to=0]
	\arrow[shorten <=9pt, shorten >=5pt, Rightarrow, no head, from=4, to=5]
	\arrow[shorten <=7pt, shorten >=7pt, Rightarrow, no head, from=6, to=4]
\end{tikzcd}\]
Now composing with an appropriate whiskering of $\rho_{u_1,u_2}^{-1}$ gives the promised identity 2-cell.
We conclude that there is an arrow $\tilde{u}_2\colon R'\to R$ in $\frakW$ such that 
diagram {\bf (II)} pre-composed with $\tilde{u}_2$ is an identity 2-cell as claimed.   When we substitute this in (\ref{number7}), we get the following pasting diagram:
% https://q.uiver.app/?q=WzAsMTIsWzAsMiwiUiciXSxbMSwyLCJSIl0sWzIsMiwiUF97dV8xXFxvdmVybGluZXt2fV8xLHVfMlxcb3ZlcmxpbmV7dn1fMn0iXSxbMywxLCJEIl0sWzIsMywiUF97dV8ydl8xXiosdV8yXFxvdmVybGluZXt2fV8yfSJdLFszLDMsIkQnIl0sWzQsMSwiQSciXSxbMywyLCJQX3t1XzEsdV8yfSJdLFs0LDMsIkEnJyJdLFs2LDIsIkIiXSxbNCwwLCJCJyJdLFs0LDQsIkInJyJdLFswLDEsIlxcdGlsZGV7dX1fMiJdLFsxLDIsInIiXSxbMiwzLCJcXHBpX0QiXSxbMSw0LCJcXHBpXzIiLDFdLFs0LDUsIlxccGknJ197RCd9IiwyXSxbMiw1LCJcXHBpX3tEJ30iLDFdLFszLDYsIlxcb3ZlcmxpbmV7dn1fMSJdLFsyLDcsIndfe3VfMSx1XzJ9Il0sWzcsNiwiXFxwaV97QSd9IiwxXSxbNyw4LCJcXHBpX3tBJyd9Il0sWzYsOSwiZl8xIiwxXSxbMywxMCwiXFxvdmVybGluZXtmfV8xIl0sWzEwLDksInZfMSIsMCx7ImN1cnZlIjotMX1dLFs1LDExLCJcXG92ZXJsaW5le2Z9XzIiLDJdLFs1LDgsIlxcb3ZlcmxpbmV7dn1fMiIsMV0sWzgsOSwiZl8yIiwxXSxbMTEsOSwidl8yIiwyLHsiY3VydmUiOjF9XSxbMTcsMTUsIiIsMSx7InNob3J0ZW4iOnsic291cmNlIjo1MCwidGFyZ2V0IjozMH0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTgsMTksIiIsMCx7InNob3J0ZW4iOnsic291cmNlIjo0MCwidGFyZ2V0IjozMH0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMjEsMjYsIiIsMix7Im9mZnNldCI6NSwic2hvcnRlbiI6eyJ0YXJnZXQiOjUwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyNCwyMiwiXFxkZWx0YV8xIiwwLHsib2Zmc2V0Ijo1LCJzaG9ydGVuIjp7InRhcmdldCI6NTB9fV0sWzIyLDI3LCJcXGJldGEiLDAseyJvZmZzZXQiOjUsInNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XSxbMjcsMjgsIlxcZGVsdGFfMl57LTF9IiwwLHsib2Zmc2V0Ijo1LCJzaG9ydGVuIjp7InNvdXJjZSI6NDB9fV1d
\[\begin{tikzcd}[ampersand replacement=\&]
	\&\&\&\& {B'} \\
	\&\&\& D \& {A'} \\
	{R'} \& R \& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \& {P_{u_1,u_2}} \&\&\& B \\
	\&\& {P_{u_2v_1^*,u_2\overline{v}_2}} \& {D'} \& {A''} \\
	\&\&\&\& {B''}
	\arrow["{\tilde{u}_2}", from=3-1, to=3-2]
	\arrow["r", from=3-2, to=3-3]
	\arrow["{\pi_D}", from=3-3, to=2-4]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi_2}"{description}, from=3-2, to=4-3]
	\arrow["{\pi''_{D'}}"', from=4-3, to=4-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi_{D'}}"{description}, from=3-3, to=4-4]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\overline{v}_1}", from=2-4, to=2-5]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{w_{u_1,u_2}}", from=3-3, to=3-4]
	\arrow["{\pi_{A'}}"{description}, from=3-4, to=2-5]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{\pi_{A''}}", from=3-4, to=4-5]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{f_1}"{description}, from=2-5, to=3-7]
	\arrow["{\overline{f}_1}", from=2-4, to=1-5]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{v_1}", curve={height=-6pt}, from=1-5, to=3-7]
	\arrow["{\overline{f}_2}"', from=4-4, to=5-5]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{\overline{v}_2}"{description}, from=4-4, to=4-5]
	\arrow[""{name=8, anchor=center, inner sep=0}, "{f_2}"{description}, from=4-5, to=3-7]
	\arrow[""{name=9, anchor=center, inner sep=0}, "{v_2}"', curve={height=6pt}, from=5-5, to=3-7]
	\arrow[shorten <=21pt, shorten >=12pt, Rightarrow, no head, from=1, to=0]
	\arrow[shorten <=15pt, shorten >=11pt, Rightarrow, no head, from=2, to=3]
	\arrow[shift right=5, shorten >=5pt, Rightarrow, no head, from=4, to=7]
	\arrow["{\delta_1}", shift right=5, shorten >=7pt, Rightarrow, from=6, to=5]
	\arrow["\beta", shift right=5, shorten <=4pt, shorten >=4pt, Rightarrow, from=5, to=8]
	\arrow["{\delta_2^{-1}}", shift right=5, shorten <=6pt, Rightarrow, from=8, to=9]
\end{tikzcd}\]
We can rewrite this as
% https://q.uiver.app/?q=WzAsMTAsWzAsMiwiUiciXSxbMSwyLCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsdV8yXFxvdmVybGluZXt2fV8yfSJdLFsyLDAsIkQiXSxbMiw0LCJEJyJdLFsyLDIsIlBfe3VfMSx1XzJ9Il0sWzMsMSwiQSciXSxbMywzLCJBJyciXSxbNCwyLCJCIl0sWzQsMCwiQiciXSxbNCw0LCJCJyciXSxbMCwxLCJyXFx0aWxkZXt1fV8yIl0sWzEsMiwiXFxwaV9EIl0sWzEsMywiXFxwaV97RCd9IiwyXSxbMSw0LCJ3X3t1XzEsdV8yfSIsMl0sWzQsNSwiXFxwaV97QSd9IiwxXSxbNCw2LCJcXHBpX3tBJyd9IiwxXSxbMiw1LCJcXG92ZXJsaW5le3Z9XzEiLDFdLFszLDYsIlxcb3ZlcmxpbmV7dn1fMiIsMV0sWzYsNywiZl8yIiwxXSxbNSw3LCJmXzEiLDFdLFszLDksIlxcb3ZlcmxpbmV7Zn1fMiIsMl0sWzIsOCwiXFxvdmVybGluZXtmfV8xIl0sWzgsNywidl8xIl0sWzksNywidl8yIiwyXSxbMTksMTgsIlxcYmV0YSIsMix7Im9mZnNldCI6NSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxMSwxNiwiIiwwLHsic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjMwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMiwxNywiIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjMwfSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyMSwxOSwiXFxkZWx0YV8xIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFsxOCwyMCwiXFxkZWx0YV8yXnstMX0iLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV1d
\[\begin{tikzcd}[ampersand replacement=\&]
	\&\& D \&\& {B'} \\
	\&\&\& {A'} \\
	{R'} \& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \& {P_{u_1,u_2}} \&\& B \\
	\&\&\& {A''} \\
	\&\& {D'} \&\& {B''}
	\arrow["{r\tilde{u}_2}", from=3-1, to=3-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi_D}", from=3-2, to=1-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi_{D'}}"', from=3-2, to=5-3]
	\arrow["{w_{u_1,u_2}}"', from=3-2, to=3-3]
	\arrow["{\pi_{A'}}"{description}, from=3-3, to=2-4]
	\arrow["{\pi_{A''}}"{description}, from=3-3, to=4-4]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\overline{v}_1}"{description}, from=1-3, to=2-4]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\overline{v}_2}"{description}, from=5-3, to=4-4]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{f_2}"{description}, from=4-4, to=3-5]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{f_1}"{description}, from=2-4, to=3-5]
	\arrow[""{name=6, anchor=center, inner sep=0}, "{\overline{f}_2}"', from=5-3, to=5-5]
	\arrow[""{name=7, anchor=center, inner sep=0}, "{\overline{f}_1}", from=1-3, to=1-5]
	\arrow["{v_1}", from=1-5, to=3-5]
	\arrow["{v_2}"', from=5-5, to=3-5]
	\arrow["\beta"', shift right=5, shorten <=4pt, shorten >=4pt, Rightarrow, from=5, to=4]
	\arrow[shorten <=11pt, shorten >=11pt, Rightarrow, no head, from=0, to=2]
	\arrow[shorten <=11pt, shorten >=11pt, Rightarrow, no head, from=1, to=3]
	\arrow["{\delta_1}"{description}, shorten <=7pt, shorten >=7pt, Rightarrow, from=7, to=5]
	\arrow["{\delta_2^{-1}}"{description}, shorten <=7pt, shorten >=7pt, Rightarrow, from=4, to=6]
\end{tikzcd}\]
If we assume that  $\beta$ is invertible, this pasting is equal to the following by definition of $w_{v_1,v_2}$ given in Section \ref{horcomppb}:
% https://q.uiver.app/?q=WzAsOCxbMCwxLCJSJyJdLFsxLDEsIlBfe3VfMVxcb3ZlcmxpbmV7dn1fMSx1XzJcXG92ZXJsaW5le3Z9XzJ9Il0sWzEsMCwiRCJdLFsxLDIsIkQnIl0sWzIsMCwiQiciXSxbMiwxLCJQX3t2XzEsdl8yfSJdLFsyLDIsIkInJyJdLFszLDEsIkIiXSxbMCwxLCJyXFx0aWxkZXt1fV8yIl0sWzEsMiwiXFxwaV9EIl0sWzEsMywiXFxwaV97RCd9IiwyXSxbMiw0LCJcXG92ZXJsaW5le2Z9XzEiXSxbMyw2LCJcXG92ZXJsaW5le2Z9XzIiLDJdLFsxLDUsIndfe3ZfMSx2XzJ9IiwyXSxbNSw0LCJcXHBpX3tCJ30iLDJdLFs1LDYsIlxccGlfe0InJ30iXSxbNCw3LCJ2XzEiLDAseyJjdXJ2ZSI6LTF9XSxbNiw3LCJ2XzIiLDIseyJjdXJ2ZSI6MX1dLFs5LDE0LCIiLDAseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEwLDE1LCIiLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE3LDE2LCJcXHJob197dl8xLHZfMn0iLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV1d
\[\begin{tikzcd}[ampersand replacement=\&]
	\& D \& {B'} \\
	{R'} \& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \& {P_{v_1,v_2}} \& B \\
	\& {D'} \& {B''}
	\arrow["{r\tilde{u}_2}", from=2-1, to=2-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\pi_D}", from=2-2, to=1-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\pi_{D'}}"', from=2-2, to=3-2]
	\arrow["{\overline{f}_1}", from=1-2, to=1-3]
	\arrow["{\overline{f}_2}"', from=3-2, to=3-3]
	\arrow["{w_{v_1,v_2}}"', from=2-2, to=2-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{\pi_{B'}}"', from=2-3, to=1-3]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{\pi_{B''}}", from=2-3, to=3-3]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{v_1}", curve={height=-6pt}, from=1-3, to=2-4]
	\arrow[""{name=5, anchor=center, inner sep=0}, "{v_2}"', curve={height=6pt}, from=3-3, to=2-4]
	\arrow[shorten <=8pt, shorten >=8pt, Rightarrow, no head, from=0, to=2]
	\arrow[shorten <=8pt, shorten >=8pt, Rightarrow, no head, from=1, to=3]
	\arrow["{\rho_{v_1,v_2}}"{description}, shorten <=5pt, shorten >=5pt, Rightarrow, from=5, to=4]
\end{tikzcd}\]
When we post-compose this with $\rho_{v_1,v_2}^{-1}$ we find that  when the pasting of diagram {\bf (I)} is pre-composed with $\tilde{u}_2$ and post-composed with $v_1$, the result is equal to the identity 2-cell on $v_1\pi_{B'}w_{v_1,v_2}r\tilde{u}_2$. 
So there is an arrow $\tilde{v}_1\colon R''\to R$ in $\frakW$ such that pasting $A$ pre-composed by $r\tilde{u}_2\tilde{v}_1$ is the identity 2-cell on $\pi_{B'}w_{v_1,v_2}r\tilde{u}_2\tilde{v}_1$.
We finally post-compose with $\gamma$ to find that when $\widetilde{\gamma\beta}$ is precomposed with $r\tilde{u}_2\tilde{v}_1$ is equal to
% https://q.uiver.app/?q=WzAsOCxbMCwxLCJSJyciXSxbMiwxLCJQX3t1XzFcXG92ZXJsaW5le3Z9XzEsdV8yXFxvdmVybGluZXt2fV8yfSJdLFszLDAsIkQiXSxbMywyLCJEJyJdLFszLDEsIlBfe3VfMSx1XzJ9Il0sWzQsMCwiQiciXSxbNCwyLCJCJyciXSxbNSwxLCJDIl0sWzAsMSwiclxcdGlsZGV7dX1fMlxcdGlsZGV7dn1fMSJdLFsxLDIsIlxccGlfRCJdLFsxLDMsIlxccGlfe0QnfSIsMl0sWzEsNCwid197dV8xLHVfMn0iLDJdLFs0LDUsIlxccGlfe0InfSIsMV0sWzQsNiwiXFxwaV97QicnfSIsMV0sWzIsNSwiXFxvdmVybGluZXtmfV8xIiwxXSxbMyw2LCJcXG92ZXJsaW5le2Z9XzIiLDFdLFs1LDcsImdfMSJdLFs2LDcsImdfMiIsMl0sWzE2LDE3LCJcXGdhbW1hIiwwLHsib2Zmc2V0Ijo1LCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV1d
\[\begin{tikzcd}[ampersand replacement=\&]
	\&\&\& D \& {B'} \\
	{R''} \&\& {P_{u_1\overline{v}_1,u_2\overline{v}_2}} \& {P_{u_1,u_2}} \&\& C \\
	\&\&\& {D'} \& {B''}
	\arrow["{r\tilde{u}_2\tilde{v}_1}", from=2-1, to=2-3]
	\arrow["{\pi_D}", from=2-3, to=1-4]
	\arrow["{\pi_{D'}}"', from=2-3, to=3-4]
	\arrow["{w_{u_1,u_2}}"', from=2-3, to=2-4]
	\arrow["{\pi_{B'}}"{description}, from=2-4, to=1-5]
	\arrow["{\pi_{B''}}"{description}, from=2-4, to=3-5]
	\arrow["{\overline{f}_1}"{description}, from=1-4, to=1-5]
	\arrow["{\overline{f}_2}"{description}, from=3-4, to=3-5]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{g_1}", from=1-5, to=2-6]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{g_2}"', from=3-5, to=2-6]
	\arrow["\gamma", shift right=5, shorten <=4pt, shorten >=4pt, Rightarrow, from=0, to=1]
\end{tikzcd}\]
\textcolor{red}{Should this be $P_{v_1, v_2}$ in the middle?}
We conclude that the diagram given in Section \ref{horcomppb} and the diagram constructed from the vertical composition of whiskerings are equivalent as claimed. 
\end{proof}
